Beyond Binary: Multiclass Paraphasia Detection with Generative Pretrained Transformers and End-to-End Models

Aphasia is a language disorder that can lead to speech errors known as paraphasias, which involve the misuse, substitution, or invention of words. Automatic paraphasia detection can help those with Aphasia by facilitating clinical assessment and treatment planning options. However, most automatic paraphasia detection works have focused solely on binary detection, which involves recognizing only the presence or absence of a paraphasia. Multiclass paraphasia detection represents an unexplored area of research that focuses on identifying multiple types of paraphasias and where they occur in a given speech segment. We present novel approaches that use a generative pretrained transformer (GPT) to identify paraphasias from transcripts as well as two end-to-end approaches that focus on modeling both automatic speech recognition (ASR) and paraphasia classification as multiple sequences vs. a single sequence. We demonstrate that a single sequence model outperforms GPT baselines for multiclass paraphasia detection.

==> media/tables/word_level_table.tex <==
\begin{table*}[t]
\caption{Word-level results aggregated over all folds. We perform statistical significance testing against GPT-3.5 and GPT-4 and represent improvements using $\dagger$ and $\ddagger$ respectively } 
    \centering
    \smaller
    \begin{tabular}{l|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{3}{c}{}  & \multicolumn{1}{|c|}{TD-binary} & \multicolumn{4}{|c}{TD-multiclass}\\
    \midrule
    Models & WER & AWER & all para & [p] & [n] & [s] & all \\ % Header row
    \midrule
    \emph{ASR Transcripts (Baseline)} &&&&&&&\\
    % \multicolumn{8}{l}{\emph{Baseline}} \\
    \hspace{15pt}GPT-3.5             & 38.6 & 32.9 & 1.17 & 1.02 & 0.67 & 0.30 & 1.99 \\
    \hspace{15pt}GPT-4               & 38.6 & \textbf{32.7} & 0.68 & 0.86 & 0.73 & \textbf{0.29} & 1.88 \\
    \midrule
    \emph{Proposed} &&&&&&&\\
    \hspace{15pt}Single-Seq          & \textbf{37.6} & 32.8 & \textbf{0.63}$\dagger$$\ddagger$ & \textbf{0.76}$\dagger$$\ddagger$ & \textbf{0.45}$\dagger$$\ddagger$ & 0.31 & \textbf{1.51}$\dagger$$\ddagger$  \\
    \hspace{15pt}Multi-Seq               & 44.8 & 42.9 & 0.86$\dagger$ & 0.90$\dagger$ & 0.72 $\dagger$ & 0.53 & 2.15 \\
    \midrule
    \emph{Oracle Transcripts} &&&&&&&\\
    \hspace{15pt} GPT-3.5          & 0.0  & 10.6 & 0.82 & 0.97 & 0.54 & 0.30 & 1.81 \\
    \hspace{15pt} GPT-4            & 0.0  & 7.9  & 0.25 & 0.67 & 0.44 & 0.27 & 1.38 \\
    \bottomrule
    \end{tabular}
    \label{tab:word-level}
\end{table*}
